Separating Technological and Clinical Safety Assurance for Medical Devices

The safety and clinical effectiveness of medical devices are closely associated with their specific use in clinical treatments. Assuring safety and the desired clinical effectiveness is challenging. Different people may react differently to the same treatment due to variability in their physiology and genetics. Thus, we need to consider the outputs and behaviour of the device itself as well as the effect of using the device to treat a wide variety of patients. High-intensity focused ultrasound systems and radiation therapy machines are examples of systems in which this is a primary concern. Conventional monolithic assurance cases are complex, and this complexity affects our ability to address these concerns adequately. Based on the principle of separation of concerns, we propose separating the assurance of the use of these types of systems in clinical treatments into two linked assurance cases. The first assurance case demonstrates the safety of the manufacturer's device independent of the clinical treatment. The second demonstrates the safety and clinical effectiveness of the device when it is used in a specific clinical treatment. We introduce the idea of these separate assurance cases, and describe briefly how they are separated and linked.

==> Sections/Benefits.tex <==
% Merits & Limitations
\section{Benefits and Limitations}
\label{merits and limitations}
		This new approach to assuring safety of medical devices provides several advantages over the traditional monolithic approach to assurance cases. 
		The primary advantage of this separation into technological and clinical ACs is that it reduces the complexity of each of the two cases. An additional benefit is that it separates out the clinical safety and effectiveness of the device in a way that does not raise questions regarding the compositionality of safety. This facilitates being able to add or modify existing clinical procedures as additional assurance cases when required, without compromising the argumentation around the system being able to deliver its outputs safely and effectively. This can significantly reduce the effort required to add compelling arguments to the safety and effectiveness of new clinical procedures the system is to be used in, reducing barriers medical companies have in being approved for new treatment methods using  existing devices. This method of separation also makes use of the idea of assurance case templates~\cite{Wassyng2015} and patterns~\cite{denney2013formal,yamamoto2013evaluation}, applied to medical devices, allowing sections of such assurance cases to be reused for modified systems or product lines. This has the potential to enable more rapid development, and ultimately approval, of medical devices.
		
		One limitation of this separation scheme that we have observed involves delimiting of which aspects relate to the technology and which relate to the clinical and how they should be dealt with in the processes most companies have already instituted. In the beginning we thought this would be easy; it was not. Until we arrived at the appropriate definitions of technological effects, technological safety, technological effectiveness, clinical effects, clinical safety and clinical effectiveness, we had consistent problems related to what belongs where. Those definitions enabled us to set rules for boundaries and relationships between the \ac{tac} and \ac{cac}.

        Another limitation is that this is approach to structuring assurance cases is new. Some manufacturers and some regulators are still working out how to handle the overall development of an assurance case for a medical system. Something new is not always welcome.

==> Sections/Preliminaries.tex <==
% Preliminaries
\section{Preliminaries}
\label{preliminaries}
	
		% Background
		\subsection{Background}
			In discussion related to assurance cases and in the structure of the assurance case figures, we have used Goal Structuring Notation (GSN)~\cite{GSNcommunityStandard2011} with some minor changes in terminology. For example, we prefer to talk about \emph{claims} and \emph{evidence} rather than \emph{goals} and \emph{solutions}.
	
		% Definitions
		\subsection{Basic Concepts}
		\label{definitions}
		
        Prior to delving into our proposed separation of assurance, we need to make an important distinction between two concepts relating to medical devices. This distinction provides a basis for our rationale for the separation of assurance discussed in \Cref{sec:proposal}.
		
			\subsubsection*{Technological effects:}
				When considering the \textit{technological effects} of the medical device, we consider the device solely as a machine that produces deterministic outputs given specific inputs. For example, a \ac{fus} machine can be viewed simply as a machine that delivers high-intensity ultrasound energy focused at a certain location in space as required by its user. Similarly, a radiation therapy machine can be viewed simply as a machine that delivers radiation energy to a certain confined location in space as required by its user. In both examples, it does not include how the output of the medical device affects patients.
			
			\subsubsection*{Clinical effects:}
            \label{clinical effects}
			    We are concerned with the use of the medical device for a particular clinical treatment, in which patient variability leads to variability in response to the outputs of the medical device. As such, \textit{clinical effects} refers to how the use of the medical device and its operating procedures can achieve the desired physiological response for the planned specific medical procedure/treatment on patients. This is meant to cope specifically with the fact that different people can react differently to the exact same treatment. In our example of the \ac{fus}, the intended clinical effects from using the device refers to how the device can be used to produce outputs, technological effects, that result in the intended biological/physiological response for the specific medical indication. This includes how the amount, focus and duration of ultrasound waveforms produced by the machine may affect a human patient. Operating procedures and treatment plans also influence the clinical effects. Pre-treatment dietary changes or medication are actions that can be taken that do not change the behaviour of the medical device and its technological effects, but may alter how the patient's body responds to the technological effects. Thus, operating procedures, pre-treatment and treatment plans are included in how we produce the intended clinical effects.

                The actual definitions of these terms and derivative terminology are shown in the relevant assurance cases in the following section on the proposed separation of assurance cases, Section~\ref{sec:proposal}.

==> Sections/RelatedWork.tex <==
% Related Work
\section{Related Work}
\label{related work}
		
		Strategies for dealing with the complexity posed by safety-critical systems for the construction of assurance cases are not new. Their software-intensive dependence often requires the specification of increasingly intricate arguments. One of the tactics to address this issue is the adoption of a compositional approach along with decomposition of the arguments into separate, but interrelated modules~\cite{kelly_using_2007,kelly_concepts_2001}. This approach provides the theoretical basis for composing our \ac{tac} and \ac{cac}. However, we are not implying that safety is compositional. We have arranged it so that the \ac{tac} and \ac{cac} are ``linked'' rather than ``composed'', by recognizing that portions of an assurance case that would be constructed in a typical monolithic structure can be arranged so that they are independent of the clinical effects of the outputs of the medical system.

		The creation of assurance case frameworks for medical device certification is something regarded as valuable, as it could facilitate the work of the manufacturers and regulatory agencies, and potentially lower the entry barrier to building assured medical devices. The conception of such frameworks would require the definition of a set of agreed argumentation patterns as a means to provide grounds for confidence in the system safety. Likewise, to diminish the barrier of assurance case adoption by the medical device community, it would be useful that regulators, such as the \ac{fda}, approve a set of templates for different types of medical devices. One of the pioneering studies that discusses the creation of assurance case frameworks for medical devices certification used generic infusion pumps as a guide to introduce these concerns~\cite{weinstock_towards_2009}.

		The decomposition of assurance cases for safety-critical systems can also be considered from the perspective of coordination of interrelated critical properties, such as system safety and security. This is especially important due to the increasing complexity of interconnected systems with new features~\cite{romanovsky_devils_2019}. Due to its prevalence and technical complexity, embedded software is a recurring example of the difficulty in assuring critical quality properties of interest. Assuring both safety and security in such systems can be onerous for both technical and social-technical reasons~\cite{aldinhas_ferreira_challenges_2022,johnson_independent_2020}.
		
		Within this perspective, a new approach of how to develop assurance cases will be beneficial, aimed at lowering the effort required for product certification. One way to accomplish this is to separate the quality attributes of interest beforehand through an independent co-assurance approach. Independent co-assurance is the conceptual shift behind maintaining separate assurance processes that contain at least two critical quality properties. This relatively recent approach to assurance has been applied in the medical domain applied to infusion pumps~\cite{romanovsky_devils_2019}, in collaborative industrial robot applications~\cite{aldinhas_ferreira_challenges_2022}, and in the automotive industry~\cite{warg_argument_2019}.

Product lines are another example of %software-intensive medical
systems where separation of concerns for assurance cases may be important.  Product lines, with many systemvariants sharing functionalities grouped in features, arise in numerous examples including pacemakers~\cite{bessling_towards_2013} and medical imaging processing tools~\cite{schwanke_experience_2004}. Depending on the particular medical application, specific application logic and intended use, medical devices product lines are categorized in product line commonalities or product line variabilities~\cite{hatcliff_challenges_2019}. On top of this, such systems must also satisfy their safety properties in all permissible settings and some of the safety artefacts should also be reusable.
		
		In our approach, the \ac{fus} can be considered a product line since there exist system components and functions that will remain the same throughout the system~\cite{hatcliff_challenges_2019}. When it is combined with \ac{mri}, the \ac{mrgfus} system promotes the possibility of treating several different medical conditions through different mechanisms of action. Such mechanisms of action can induce different biological effects~\cite{noauthor_foundation_2021} into the patient's body to produce a variety of biological/physiological responses. Therefore, the existing different behaviours that a \ac{fus} machine can produce configures product lines since it aims at delivering customized treatment for a single patient or a predefined range of patients based on their pre-existent medical condition. There are many challenges posed in the development of assurance cases for a product line family with a proper separation of concerns regardless of the domain to which it belongs. As the system evolves, complexity may be added to the development of assurance cases since more solution options (product line) are made available. This kind of issue has been approached before for the construction of complete product-line assurance cases for all possible variants that might be derived from a product line, but actually without performing these derivations~\cite{nesic_product-line_2021}.

